FLAME: A Fast Large-scale Almost Matching Exactly Approach to Causal Inference

A classical problem in causal inference is that of matching, where treatment units need to be matched to control units based on covariate information. In this work, we propose a method that computes high quality almost-exact matches for high-dimensional categorical datasets. This method, called FLAME (Fast Large-scale Almost Matching Exactly), learns a distance metric for matching using a hold-out training data set. In order to perform matching efficiently for large datasets, FLAME leverages techniques that are natural for query processing in the area of database management, and two implementations of FLAME are provided: the first uses SQL queries and the second uses bit-vector techniques. The algorithm starts by constructing matches of the highest quality (exact matches on all covariates), and successively eliminates variables in order to match exactly on as many variables as possible, while still maintaining interpretable high-quality matches and balance between treatment and control groups. We leverage these high quality matches to estimate conditional average treatment effects (CATEs). Our experiments show that FLAME scales to huge datasets with millions of observations where existing state-of-the-art methods fail, and that it achieves significantly better performance than other matching methods.

==> CoverLetter.tex <==
Dear Editors,

Please find our manuscript "FLAME: A Fast Large-scale Almost Matching Exactly Approach to Causal Inference" for submission to JMLR. 

Appropriate editors might include Edoardo Airoldi and Russ Greiner.

We need to let you know that we have a conflict of interest with editors Mehryar Mohri, David Sontag, and Joris Mooij. We also have a conflict with Nathan Kallus, who should not be chosen as a reviewer. Thank you!

This paper is related to causal inference and machine learning. We hope to get reviewers who are more open-minded to a machine learning perspective than the classical causal inference reviewers. Thank you for considering our manuscript.

This paper has not been published as a conference proceedings. Extensions of the FLAME algorithm have been published as conference proceedings, but the methods have been substantially different, and have cited the FLAME algorithm appropriately. The extensions are: (1) Dieng et al., Interpretable Almost-Exact Matching for Causal Inference. AISTATS, 2019. This paper presents a different optimization method for the optimization problem presented in the FLAME paper. The method in Dieng et al doesn't scale nearly as well as FLAME does, but it produces higher quality solutions in some cases. (2) Awan et al., Interpretable Almost-Exact Matching With Instrumental Variables. UAI, 2019. This paper presents an extension of FLAME to instrumental variables. (3) Awan et al. 2019 (in submission) extends FLAME to the case of experimental settings on networks. (In contrast, FLAME is designed for observational settings with data that has standard covariates.) The MALTS algorithm of Parikh et al, 2019, is not an extension of FLAME, it is designed for continuous covariates. Parikh et al. 2019 did combine MALTS with FLAME to produce a more powerful method that can handle mixed data.


Sincerely,
The authors

==> CoverLetterForModification.tex <==
Dear Russ,
Thank you once again for handling our paper JMLR-19-853.
We need to let you know that we found a minor error in Proposition 2. We fixed the statement and the proof in the attached version (which is also on arxiv). Sorry about the error. The statement and proof have been made more precise and this does not affect the algorithm proposed in the paper or any of the main results. Proposition 2 continues to provide the same guidance for the main algorithm, just in a more compact way.

Thanks,
Tianyu, Marco, Usaid, Yameng, Sudeepa, Cynthia, and Alex

==> algorithms.tex <==
% !TEX root = JASA-main.tex
%{
%\section{Sudeepa-- new Defn MQ}

\section{The FLAME Algorithm and Efficient Implementations}\label{sec:algorithms}
In this section, first we provide a generic FLAME algorithm called \textit{FlameGeneric} incorporating the ideas described in the previous section (Section~\ref{sec:algo-generic}).
%(Section~\ref{sec:algo-generic}). 
%Since looking at all possible partitions of the set of variables is computationally expensive, we use a greedy approach to dropping variables one by one that optimizes the objective  function in (\ref{equn:opt}). Then 
We outline two efficient implementations of the matching procedure used in this generic algorithm: (a) using a database management system and database queries (Section~\ref{sec:algo-db}), and (b) using bit vectors (Section~\ref{sec:algo-bit}).
We also discuss a faster but less adaptable variant of the generic FLAME algorithm (Section~\ref{sec:faster_flame}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Basic FLAME
% \begin{algorithm}[tb] 
\begin{algorithm}
    % \STATE{\bfseries Input:}{Input}{Input}
    % \SetKwInOut{Output}{Output} 
\begin{algorithmic} 
    \STATE  \textbf{Input:} 
    { (i) data $D=(X,Y,T)$. (ii) holdout training set $D^H=(X^H, Y^H, T^H)$. } 
    \STATE  \textbf{Output:} { A set of matched groups $\{\MG_\iter \}_{\iter \geq 1}$ and ordering of covariates $j_1^*,j_2^*,..,$ eliminated.}
    \STATE Initialize $D_0 = D = (X,Y,T),J_0=\{1,...,p\},\iter=1, run=True$, $\MG = \emptyset$. \COMMENT{\small ($\iter$ is the index for iterations, $j$ is the index for covariates)}
    \STATE $(D_0^m,D_0\setminus D_0^m, \MG_1) = \BasicExactMatch(D_0, J_0)$.
    \WHILE{$run=True $\text{ and } $D_{\iter-1}\setminus D_{\iter-1}^m \neq \emptyset$ { \texttt{ \small (we still have data to match)}}  }  \label{step:while}
        \STATE $D_{\iter} = D_{\iter-1}\setminus D_{\iter-1}^m$ \texttt{\small (remove matches)}
        \FOR{$j\in J_{\iter-1}$ \texttt{ \small (temporarily remove one feature at a time and compute match quality)}}{\label{step:1} } 
            \STATE $(D_\iter^{mj},D_\iter\setminus D_\iter^{mj}, \MG_{temp}^j) = \BasicExactMatch(D_\iter,J_{\iter-1}\setminus j)$.
            \STATE $D^{Hj}=[X^H(:,J_{\iter-1}\setminus j),Y^H,T^H]$
    	    \STATE $q_{\iter j} = \MQ(D_\iter^{mj},D^{Hj})$ 
    	\ENDFOR
    	\IF{\textrm{\rm other stopping conditions are met},\label{step:otherstopping}}
    	   \STATE $run=False$ \texttt{\small (break from the {\bf while} loop)}
        \ENDIF
        \STATE 	$j^{\star}_\iter\in \arg\min_{j\in J_{\iter-1}}q_{\iter j}$: \texttt{\small (choose feature to remove)} %, break ties using $\pi^{\textrm{lasso}}$)}
    % 	 \label{step:removefeatureselect}
    	\STATE $J_\iter=J_{\iter-1}\setminus j^{\star}_\iter$ (\texttt{\small remove feature} $j^{\star}_{\iter}$) \label{step:removefeature}
    	\STATE $D_\iter^m = D_\iter^{mj^\star}$ and $\MG_\iter =  \MG_{temp}^{j^{\star}_\iter}$ \texttt{\small (newly matched data and groups)} \label{step:newmatch} 
    	\STATE $\iter = \iter+1$
    \ENDWHILE
    \STATE \textbf{RETURN} {$\{ \MG_\iter, D_\iter^m,J_\iter \}_{\iter \geq 1}$ \texttt{\small (return all the  matched groups and covariates used)} }
\end{algorithmic}
    \caption{Generic FLAME Algorithm: \textit{FlameGeneric} }
    \label{algo:basic-FAME} 
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BasicExactMatch
\begin{algorithm}[t]
\begin{algorithmic}[1]
    \STATE{\textbf{Input: }} Unmatched Data $D^{um} =(X,Y,T)$, subset of indexes of covariates $J^s \subseteq\{1,...,p\}$.
    \STATE{\textbf{Output: }} Newly matched units $D^m$ using covariates indexed by $J^s$ where groups have at least one treatment and one control unit, the remaining data as $D^{um} \setminus D^m$ and matched groups for $D^m$.
    \STATE $M_{raw}$=\texttt{group{-}by} $(D^{um}, J^s)$. \\
    ({\tt form groups by exact matching on $J^s$}) \label{step:basic-1} \\
    \STATE $M$=\texttt{prune}($M_{raw}$) 
    ({\tt remove invalid all-treatment or all-control groups}) \label{step:basic-2} \\
% %    Attach a group-id to each group of $M$\\
    \STATE $D^m$=Get subset of $D^{um}$ where the covariates match with $M$ \texttt{\small (recover newly matched units)}\label{step:basic-3}
    \STATE \textbf{RETURN}{$\{D^m, D^{um} \setminus D^m, M\}$.}
\end{algorithmic}
    \caption{\BasicExactMatch\ procedure}
    \label{algo:basicExactMatch}
\end{algorithm}


\subsection{The Generic FLAME Algorithm}\label{sec:algo-generic}
Algorithm~\ref{algo:basic-FAME} presents the generic matching algorithm \textit{FlameGeneric} for FLAME. Initially, the input with $n$ units is given as $D = (X, Y, T)$, where %$id$ (an $n \times 1$ vector) denotes the unique identifiers of the units, 
$X$ (and $n \times p$ matrix) denotes the covariates, $Y$ (an $n \times 1$ vector) is the  outcome, and $T$  (an $n \times 1$ vector) is the treatment. The covariates are indexed with  $J = 1, \cdots, p$. 
\par
At iteration $\iter$ of the algorithm, it computes a subset of the matched groups $\MG_{\iter}$ such that for each matched group $\mg \in \bigcup_{\iter}\MG$, there is at least one treated and one control unit. Note that it is possible for $\MG_{\iter} = \emptyset$, in which case no matched groups are returned in that iteration.  Recall from the previous section that $M_u$ denotes the iteration when a unit $u$ is matched. Overloading notation, let $M_\mg$ denote the iteration when a matched group $\mg$ is formed. Hence if a unit $u$ belongs to a matched group $\mg$, $M_u = M_\mg$ (although not every $u$ with $M_u=M_{\mg}$ is in $\mg$). 
 %For a matched group $mg \in \MG$, $J_\mg \subseteq J$ denotes the set of the indexes of the covariates that are used in forming $\mg$; for two different matched groups returned in the same iteration, $J$
% If the index of the dropped covariate at iteration $\iter$ is $\pi(i)$, then all the matched groups in $\MG_i$ use covariates with indexes $J \setminus \{\pi(i)_{i=1}^{j-1}\}$, and have different combination of values of these covariates.
 \par

%{\bf Pre-computation of variable importance using lasso path:}  
%As discussed above, we use the regularization path from lasso regression of $Y$ on $[X,T]$ to construct $\pi^{lasso}$, the order in which variables vanish along the lasso path.

%As discussed above, we compute the lasso path for a single regression on $[X,T]$ with outcome $Y$, w, and pre-compute an ordering $\pi^{lasso}$ on variables. As regularization increases, features are eliminated in order of $\pi^{lasso}$ if there is a tie for variable selection for elimination inside the while loop.
%so that $\pi(j)=1$ for the covariate $j$ that vanishes first.
We use $D_{\iter} \subseteq D$ to denote the unmatched units and $J_{\iter} \subseteq J$ to denote the remaining variables when iteration $\iter+1$ of the while loop starts (\ie, after iteration $\iter$ ends). Initially $J_0 = J$. As discussed in Section~\ref{sec:fame-framework}, the algorithm drops one covariate  $\pi(\iter)$ in each iteration (whether or not there are any valid non-empty matched groups), and therefore, $J_{\iter} = J \setminus \{\pi(j)_{j=1}^{\iter}\}$, $|J_{\iter}| = p - \iter$. All matched groups $\mg \in \MG_{\iter}$ in iteration $\iter$ use $J_{\iter-1}$ as the subset of covariates on which to match. %\textcolor{red}{Is the indexing correct here?} 
\par
%{\bf Computing variable importance using Lasso path:} In the first step of Algorithm~\ref{algo:basic-FAME}, we pre-compute a measure of variable importance using the Lasso path on the holdout set $D^H$.
%\par
{\bf The first call to \BasicExactMatch:} First we initialize the variables $D_0, J_0$, $\iter$, and $run$. The variable $run$ is true as long as the algorithm is running, while $\iter \geq 1$ denotes an iteration. After the initialization step, the subroutine \BasicExactMatch\ (see Algorithm~\ref{algo:basicExactMatch}) finds all of the exact matches in the data $D = D_0$ using \emph{all} features $J = J_0$, such that each of the matched groups $\mg \in \MG_1$ contains at least one treatment and one control observation. 
%This first call to \BasicExactMatch\ returns the highest quality matches, since the treatment and control observations are matched on all of the covariates. 
%The matches returned by this first call to  \BasicExactMatch\ are `complete' in the sense that all matched groups $\mg \in \MG_1$, the entire set of covariates $J_0 = J$;  t
The rest of the iterations in the algorithm aim to find the best possible matches for the rest of the data by selectively dropping covariates as discussed in the previous section.

{\bf The while loop and subsequent calls to \BasicExactMatch:} At each iteration of the \textbf{while} loop, each feature is temporarily removed (in the \textbf{for} loop over $j$) and evaluated to determine if it is the best one to remove by running \BasicExactMatch\ and computing the matched quality $\MQ$. Since \BasicExactMatch\ does not consider feature $j$ (one less feature from the immediately previous iteration), there are fewer constraints on the matches, and it is likely that there will be new matches returned from this subroutine. 

We then need to determine whether a model that excludes feature $j$ provides sufficiently high quality matches and predictions. We would not want to remove $j$ if doing so would lead to poor predictions or if it led to few new matches. 
%Also we would not want to remove $j$ if very few new matches were created by removing it. The match quality function \MQ\ (see equation (\ref{equn:MQ}) in Section \ref{Subsec:MQ}) takes into account these criteria (performed on a holdout set). 
Thus, \MQ is evaluated by temporarily  removing each $j$, and the $j^*$ that is chosen for removal creates the most new matches 
%(proportionally to the size of treatment and control groups) 
and also does not significantly reduce the prediction quality. 
Steps \ref{step:removefeatureselect} and \ref{step:removefeature} of the algorithm choose which feature to remove, and remove it. In Step~\ref{step:newmatch}, the new matches and matched groups are stored.
%(by running \BasicExactMatch\ again after removing the chosen feature and setting the corresponding \ismatched\ values to 1). 
The remaining unmatched data %(with \ismatched\ = 0) 
are used for the next iteration $\iter+1$. 


{\bf Stopping conditions:} If we run out of unmatched data, the algorithm stops (Step~\ref{step:while}). If we choose to include another stopping condition, then we also stop (Step~\ref{step:otherstopping}). For instance, if the unmatched units are either all control or all treatment observations, we must stop. If there are no more covariates to drop, we also stop. We could also choose to stop when the match quality is too low. 
Finally, the matched groups are returned along with the units and the features used for each set of matched groups formed in different iterations.

The key component in the \textit{FlameGeneric} algorithm (Algorithm~\ref{algo:basic-FAME}) is the \BasicExactMatch\ procedure (Algorithm~\ref{algo:basicExactMatch}). The steps of \BasicExactMatch\ can be easily implemented in Java, Python, or R. In Section \ref{Sec:BEM} we give efficient implementations of  \BasicExactMatch, one using SQL queries from databases, and the other using bit vector techniques.




\subsection{Faster Feature Selection}\label{sec:faster_flame}

One could precompute the order  $\pi$ in which features are removed in FLAME. This would allow FLAME to run faster at the expense of making it less adaptable. To precompute $\pi$, we could use Lasso's regularization path or another backwards selection method to determine the order in which to remove the features before we do any matching or removing of data. This would remove lines 5-9 of the Generic FLAME algorithm, and change lines 13-14 to remove the predetermined next feature. The problem with precomputing $\pi$ is that it may choose the wrong feature to remove, since it takes into account the full dataset, but does not take into account the data that remain at the iteration when that feature is scheduled to be removed. 

If we consider a dataset that has a large number of irrelevant features, it might be beneficial to use Lasso or another technique to choose a pre-determined order to omit the clearly irrelevant features, which provides a computational gain. After that, we can switch back to the Generic FLAME implementation (including the backwards selection loop) to continue removing features.

% \subsection{Conditional Average Treatment Effect on a Sub-population} 
% Since FLAME gives the personalized treatment effect $\tau_u$ of every matched unit, we can compute treatment effects with respect to a sub-population. For example, for a sub-population with $\mathbf{X} \in \{ \mathbf{x}_1,  \dots, \mathbf{x}_g\}$ where $x_i$ is a combination of covariates, the \emph{conditional average treatment effect on the treated} (CATT) is estimated by 
% \begin{align*}
%     \text{CATT}(\mathbf{X}) = \frac{1}{\#\{u:T_u=1,X_u\in\mathbf{X}\}}\sum_{u: T_u=1,X_u\in \mathbf{X}}\tau_u
% \end{align*}
% For estimating the \emph{conditional average treatment effect} (CATE)

% % \begin{align}
% % \text{CATT}(  \mathbf{X} \in \{ \mathbf{x}_1, \dots, \mathbf{x}_g \} ) = \frac{ \sum_{i=1}^{g} S^t(\mathbf{x}_i) \left( O^t (\mathbf{x}_i) - O^c (\mathbf{x}_i) \right) }{ \sum_{i=1}^{g} S^t(\mathbf{x}_i)  } \label{eq:catt}
% % \end{align}
% % where $O^c (\mathbf{x}_i)$ ($O^t (\mathbf{x}_i) $) is the average outcome of the control (treated) units whose variable values are $\mathbf{x}_i$, $S^t(\mathbf{x}_i)$ is the number of treated units whose variable values are $\mathbf{x}_i$. 
% With this formula, we can compute CATT of any sub-population of interest. To estimate the \emph{conditional average treatment effect} (CATE) using the same equation we require a further assumption that the treatment and control covariate distributions are the same. Alternatively, one can construct a sequence of matches


% If we assume that the treated population and the control populations are similar, we can estimate \emph{conditional average treatment effect} (CATE) of any sub-population by replacing $S^t(\mathbf{x}_i)$ with the number of both treated and control units whose variable values are $\mathbf{x}_i$ in (\ref{eq:catt}). In particular, we can estimate the overall CATT or CATE by letting $\{ \mathbf{x}_1, \dots, \mathbf{x}_G \}$ be the set of all possible variable values in the whole population. As an example, if we assume the treated population and the control population are similar, then the overall CATE is estimated by
% \begin{align*}
% \text{CATE} &= \text{CATE}(  \mathbf{X} \in \{ \mathbf{x}_1, \dots, \mathbf{x}_G \} ) \\
% &= \frac{ \sum_{i=1}^{G} S(\mathbf{x}_i) \left( O^t (\mathbf{x}_i) - O^c (\mathbf{x}_i) \right) }{ \sum_{i=1}^{G} S(\mathbf{x}_i)  }
% \end{align*}
% where $S(\mathbf{x}_i)$ is the number of treated and control units whose variables values are $\mathbf{x}_i$
% %We can also incorporate inverse of the variance of the outcomes in the groups into the estimated ATT. The variance quantifies uncertainty.
% %\red{Write about both CATE and CATT -- at the end generalize to the full population}



==> causal_forests/cf.tex <==
\section{FLAME and Causal Forests}
The  Causal Forests algorithm \citep{wager2018estimation, athey2019generalized} is a method that learns both a model for the counterfactuals and one for the propensity. While Causal Forests are used to estimate CATEs, the method should not be interpreted as a matching method. In this section we compare FLAME to Causal Forests and show that:
\begin{enumerate}
    \item While Causal Forests can technically be interpreted as a matching method, according to a very broad definition of matching, the matches it produces are almost always uninterpretable.
    \item Causal Forests produce ``matches'' of either similar or lower quality than FLAME.
\end{enumerate}
% Considering our result, there seems to be no reason to prefer Causal Forests to FLAME for the purposes of matching. 

% focus on investigating the following questions: 
% \begin{itemize}
%     \item Can we interpret causal forest \citep{} as a matching algorithm?
%     \item How well does causal forest perform in terms of matching quality, comparing to DAME \citep{} and FLAME?
% \end{itemize}


\subsection{Evaluating Causal Forest as a matching method}
In this section only, we define ``matching methods'' to mean those methods that use only a subset of units to estimate to estimate CATEs (in practice this is essentially a subgroup analysis method). In that sense one can count the number of units a unit is matched with.
% We can adopt a very broad definition of matching method, and say that an algorithm is a matching method if \textbf{it uses only a subset of units to inform CATE predictions for a single unit}. 
One top desiderata of a matching method is that one unit should not be matched to too many other units. If a unit is matched to too many others, then the match will cease to be interpretable. %\textbf{If a unit is matched to too many other units interpretability is lost}. %Clearly, if the CATE for a unit is predicted using information from hundreds of others, a human observer would have a hard time attributing that prediction to a few clear units. Because of this, the matches are uninterpretable. \\

%In this section, we compare Causal Forests to FLAME on the following criteria: how many times each unit is used in predicting the treatment effect. In the experiments, we use the following model to generate synthetic data, for each unit $i$:

%\todo{Do section 6.1.2 exactly}
In this section, we compare Causal Forests to FLAME on the number of units used in predicting the CATE for each unit. In the experiments, we use the same model as in Section \ref{sec:experiments} to generate synthetic data, for each unit $i$:
\begin{align*}
    y_i = \sum_{j}^{p} \alpha_j x_{ij} + T \sum_{j=1}^{p} \beta_j x_{ij} + T_i\cdot U \sum_{j,\gamma,\gamma>j}  x_{ij} x_{i\gamma}, 
\end{align*}
where $i$ indexes units and $j$ indexes covariates, $\alpha_j$ is a baseline effect of each covariate, $\beta_j$ is the treatment effect conditional on covariate $j$. The model also includes a nonlinear interaction effect between covariates: $x_jx_{\gamma}$, where each covariate interacts with all the covariates that succeeds it. This term is weighted by the coefficient $U$.

We simulate data from a model with 1000 treatment and 1000 control units, and 12 covariates, with 10 important and 2 unimportant (i.e., such that $\alpha_j, \beta_j = 0$). We implement causal forests with 200 trees and 1000 training samples per tree. We focus on estimating the CATE for each unit. 
% In this set of experiments, we summarize the results of causal forest in the following fashion: How many times each unit contributes to its prediction. If for each unit, all other units contribute at least once to its prediction, then we can not interpret causal forest as a matching algorithm.
% \subsection{Experiment Setting} 
% Nonlinear Model:

% 1000  treatment / control units

% 10 important covariates, 2 unimportant covariates

% Causal Forest 200 trees, 1000 training samples / tree

\subsubsection{Results 1: Comparison by Size of Match Group }
% In Figure~\ref{fig:cf_heat}, we can find that some pairs of units between which there are no contributions(around 60.2\% pairs of units have no contributions). So we can interpret causal forest as a matching algorithm.
% \begin{figure}[]
% \centering
% \includegraphics[width=.8\linewidth]{causal_forests/cf_heat_map.png}
% \caption{Contributions to Predictions Between Each Pair of Unit}
% \label{fig:cf_heat}
% \end{figure}
%Our first result is that for around 60.2\% of units don't contribute in estimating every CATE. This implies that causal forest does only use certain subsets of units when making CATE predictions, and, therefore, can be technically considered a matching method. We will also see shortly that, while technically a matching method, Causal Forests matches each unit to too many other units, and therefore produces uninterpretable matches.

\textcolor{red}{First, we find that 60.2\% of units do not contribute towards estimating every CATE when using causal forest. This implies that causal forest uses subsets of units when making CATE predictions, and, therefore, can be technically considered a matching method.} Second, we show in Figures \ref{fig:total_matched_both} and \ref{fig:comp_total_matched} that Causal Forests matches each unit to too many other units, and therefore produces uninterpretable matches. %We will also see shortly that, while technically a matching method, Causal Forests matches each unit to too many other units, and therefore produces uninterpretable matches.
Figure \ref{fig:total_matched_both} and \ref{fig:comp_total_matched} compare the number of units contributing to the CATE prediction for each unit. We observe that Causal Forest matches each unit to 800 other units, on average, to predict CATEs. Whereas, FLAME uses fewer than 30 units, on average. 

%FLAME uses, on average, much fewer units to make a CATE prediction than Causal Forests (less than 30 on average). The latter uses an average of close to 800 units to predict the CATE for a single unit: attributing a prediction to a small set of observations or even a single one is nearly impossible in this setting, and therefore Causal Forest matches are uninterpretable.  

\begin{figure}[H]
\centering
\begin{minipage}[b]{0.8\linewidth}
\includegraphics[width=\textwidth]{causal_forests/hist_matched_grp_units_flame.png}
\end{minipage}
\caption{Histogram of number of units used to predict each CATE.}
\label{fig:total_matched_both}
\end{figure}

\begin{figure}[H]
\centering
\begin{minipage}[b]{0.8\linewidth}
\includegraphics[width=\textwidth]{causal_forests/compare_matched_grp_units_flame.png}
\end{minipage}
\caption{Number of observations contributing to each CATE prediction: Causal Forest vs. FLAME. Each dot is a CATE for one unit's matched group, the $x$ axis shows the number of units that contribute to the prediction for that CATE for Causal Forests, and the $y$ axis for FLAME.}
\label{fig:comp_total_matched}
\end{figure}

\subsection{Matching Quality for Causal Forest and FLAME}
In this experiment, we compare matching quality of causal forest and FLAME by looking at the average hamming distance between each unit and all other units that contribute to its prediction. The \textbf{Average Hamming Distance (AHD)} for each unit $i$ is defined as:

\begin{equation}
\mbox{AHD}_i = \frac{\sum_j\mbox{HammingDistance}(i, j)}{|\mbox{ContributionSet}_i|} \quad \forall j \in \mbox{ContributionSet}_i\\,
\end{equation}
where \textbf{Contribution Set} for unit $i$ as per FLAME is defined as all units in its \textbf{main matched group} and as per Causal Forests it is defined as all units in all leaves used to predict CATE for unit $i$. $|\mbox{ContributionSet}_i|$ denotes the cardinality of the Contribution Set for unit $i$. We show that Causal Forests achieves lower average match quality than FLAME in our setting. 

This experiment was performed with the same outcome model, and parameters as the previous one, but this time there are 10 important covariates and 5 unimportant ones. In addition, we early-stop FLAME when matching quality drops by 5\%, so FLAME runs totally 9 iterations. 

%as ``\textbf{out-of-bag}" predictions for unit $i$
% \subsection{Experiment Setting}
% Nonlinear Model:

% $y = \sum_{i}^{} \alpha_i x_i + T \sum_{i=1}^{} \beta_i x_i + T\cdot U \sum_{i,\gamma,\gamma>i}  x_i x_{\gamma}$

% 1000  treatment / control units

% 5 important covariates, 10 unimportant covariates

% Causal Forest 200 trees, 1000 training samples / tree

% For FLAME, we early-stop the algorithm when matching quality drops by 5\%, so FLAME runs totally 9 iterations. 

\subsubsection{Results 2: Comparison in Unit-level Average Hamming Distance}
Figure~\ref{fig:comp_unit_ahd_colors} shows the average hamming distance between each unit and its matched group in both algorithms. The blue line in the plot represent the 45 degree line. As we can see, there are much more units below the 45 degree line (495) than above the line (127). This indicates that there are more units which have larger average hamming distance (or lower matching quality) in Causal Forest than in FLAME. We can conclude that FLAME generates better unit-level matching quality than Causal Forest.

Units in Figure \ref{fig:comp_unit_ahd_colors} are color-coded according to which iteration of FLAME they were matched at. This shows that the hamming distances of units matched by FLAME, i.e., the matching quality of FLAME, tends to degrade while dropping covariates. This is expected and consistent with our theoretical and experimental results for FLAME.

\begin{figure}[!ht]
\centering
\begin{minipage}[b]{0.8\linewidth}
\includegraphics[width=\textwidth 
]{causal_forests/avg_hamming_dist_colors_small.png}
\end{minipage}
%avg_hamming_dist_colors_small
\caption{Comparison of Unit-level Average Hamming Distance with Colors. Each dot is a unit. The $x$ axis represents matched quality for the Causal Forests matched group of each unit, and the $y$ axis matched quality for the FLAME matched group of each unit.}
\label{fig:comp_unit_ahd_colors}
\end{figure}

\subsubsection{Results 3: Comparison in Group-level Average Hamming Distance}
We investigate how the amount of units used for each match affects match quality. We divide units into groups, where a ``group" contains all units with same size matched group. The \textbf{Group-Level Average Hamming Distance (G-AHD)} is defined as:

\begin{equation}
\mbox{G-AHD}_i = \frac{\sum_j\mbox{AHD}_j} {|\mbox{Group}_i|} \forall j \in \mbox{Group}_i
\end{equation}

	\begin{figure}[H]
		%\caption{Share of the different types of patents per year}
		\begin{minipage}[b]{0.5\linewidth}
			\centering
			%\textbf{Walk}\par\medskip
 			\includegraphics[width=8cm,height=8cm,keepaspectratio]{causal_forests/hamming_dist_cf_small.png}
		\end{minipage}
		\hfill		
		\begin{minipage}[b]{0.5\linewidth}
			\centering
			%\textbf{Ricksahaw}\par\medskip
			\includegraphics[width=8cm,height=8cm,keepaspectratio]{causal_forests/hamming_dist_flame.png}
		\end{minipage}

 		\caption{Comparison of Group-level Average Hamming Distance between FLAME and Causal Forest.}
        \label{fig:grp_ahd_flame_cf}
	\end{figure}



%Figure \ref{fig:grp_ahd_cf_flame} and \ref{fig:grp_ahd_dame_flame} show the results for group-level average hamming distance.
Figure \ref{fig:grp_ahd_flame_cf} shows the results for group-level average hamming distance for Causal Forest and FLAME. Figure~\ref{fig:grp_ahd_dame_large_flame} is an enlarged version of right panel of Figure \ref{fig:grp_ahd_flame_cf}. Different colors represent different group-level average hamming distances. We observe that FLAME generates smaller average hamming distance than causal forest. Moreover, causal forest generates large average hamming distance (or poor matching quality) for small matched groups, while FLAME generates small average hamming distance (high-quality matching) on smaller groups. This is because in causal forest a larger matched group corresponds to a large set of samples from many trees with different set of matched covariates. %, which indicates better matching quality. 
FLAME, however, still maintains high-quality matches while dropping covariates. 



%\begin{figure}[]
%\centering
%\includegraphics[width=\textwidth]{causal_forests/hamming_dist_cf_small.png}
%\caption{Comparison of Group-level Average Hamming Distance between FLAME and Causal Forest. %Each dot is a unit. The $x$ axis represents matched quality for the Causal Forests matched group of each unit, and the $y$ axis matched quality for the FLAME matched group of each unit.
%}
%\label{fig:grp_ahd_cf_flame}
%\end{figure}


%\begin{figure}[]
%\centering
%\includegraphics[width=\textwidth]{causal_forests/hamming_dist_flame.png}
%\caption{Group-level Average Hamming Distance: FLAME}
%\label{fig:grp_ahd_dame_flame}
%\end{figure}


\begin{figure}[H]
\centering
\begin{minipage}[b]{0.5\linewidth}
\includegraphics[width=\textwidth]{causal_forests/hamming_dist_flame_small.png}
\end{minipage}
\caption{Group-level Average Hamming Distance: FLAME}
\label{fig:grp_ahd_dame_large_flame}
\end{figure}
%hamming_dist_cf_small


% \begin{comment}
% \section{Matching Quality: Causal Forest VS DAME}
% In this experiment, we compare the matching quality of causal forest and DAME by looking at the average hamming distance between each unit and all other units that contribute to its prediction. 

% Here \textbf{Contribution Set} for unit $i$ in DAME is defined as:

% DAME: all units in each unit $i's$ \textbf{main matched group}

% \subsection{Experiment Setting}
% Nonlinear Model:

% $y = \sum_{i}^{} \alpha_i x_i + T \sum_{i=1}^{} \beta_i x_i + T\cdot U \sum_{i,\gamma,\gamma>i}  x_i x_{\gamma}$

% 10000  treatment / control units

% 5 important covariates, 10 unimportant covariates

% Causal Forest 200 trees, 10000 training samples / tree

% \subsection{Results 1: Size of Contribution Set}
% In Figure ~\ref{fig:total_matched_both} and ~\ref{fig:comp_total_matched}, we compare size of contribution set for each unit. As we can see, DAME has on average smaller contribution sets than causal forest.

% \begin{figure}[]
% \centering
% \includegraphics[width=\textwidth 
% ]{causal_forests/hist_matched_grp_units.png}
% \caption{Distribution of Size of Contribution Set}
% \label{fig:total_matched_both}
% \end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=\textwidth]{causal_forests/compare_matched_grp_units.png}
% \caption{Number of Total Matched Units: Causal Forest VS DAME}
% \label{fig:comp_total_matched}
% \end{figure}

% \subsection{Results 2: Comparison in Unit-level Average Hamming Distance}
% Figure~\ref{fig:comp_unit_ahd_colors} shows the average hamming distance for each unit in both algorithms. The blue line in the plot represent the 45 degree line. As we can see, there are much more units below the 45 degree line(18998) than above the line(853). This indicates that there are more units which have larger average hamming distance(or lower matching quality) in causal forest than in DAME. So DAME generates better unit-level matching quality than causal forest.

% \begin{figure}[]
% \centering
% \includegraphics[width=\textwidth ]{FLAME/causal_forests/avg_hamming_dist_colors.png}
% \caption{Comparison in Unit-level Average Hamming Distance with Colors}
% \label{fig:comp_unit_ahd_colors}
% \end{figure}

% \subsection{Results 3: Comparison in Group-level Average Hamming Distance}
% We also want to compare group-level average hamming distance.Figure~\ref{fig:grp_ahd_cf} and ~\ref{fig:grp_ahd_dame} show the results for group-level average hamming distance. Figure~\ref{fig:grp_ahd_dame_small} is an enlarged version of Figure~\ref{fig:grp_ahd_dame}. Different colors represent different group-level average hamming distance. As we can see, DAME still generates smaller average hamming distance than causal forest in general. Moreover, causal forest generates very large average hamming distance(or poor matching quality) on groups with small contribution sets, while DAME generates small average hamming distance(high-quality matching) on groups with small contribution sets. This is because in causal forest a larger contribuition set represents a larger set of samples from more trees with different set of matched covariates, which indicates better matching quality. DAME, however, matches units while dynamically dropping covariates. When more covariates are dropped, DAME matches on more units with degraded matching quality. 

% \begin{figure}[]
% \centering
% \includegraphics[width=\textwidth]{FLAME/causal_forests/hamming_dist_cf.png}
% \caption{Group-level Average Hamming Distance: Causal Forest}
% \label{fig:grp_ahd_cf}
% \end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=\textwidth]{FLAME/causal_forests/hamming_dist_dame.png}
% \caption{Group-level Average Hamming Distance: DAME}
% \label{fig:grp_ahd_dame}
% \end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=\textwidth]{FLAME/causal_forests/hamming_dist_dame_small.png}
% \caption{Group-level Average Hamming Distance: DAME}
% \label{fig:grp_ahd_dame_small}
% \end{figure}
% \end{comment}

\subsection{Conclusion}
We have shown that if one were to interpret Causal Forests as a matching algorithm, it would generate matches with poor match quality, particularly in comparison to methods like FLAME that match almost exactly. 
Causal Forests also tends to match units to a large number of other units, making the matches hard to interpret. 
%For these reasons, FLAME appears to be a better choice of method for the purposes of matching. 


==> discussion_old.tex <==
% !TEX root = JMLR-main.tex
\section{Discussion}\textcolor{red}{MOVE ME}
In this paper we introduced FLAME, an algorithm for covariate based matching in observational studies. 
\begin{itemize}[leftmargin=*]
\itemsep0em%
	\item It provides a method for approximating the gold-standard performance of exact matching.
	\item Its efficiency stems from careful bit-vector operations and specialized database queries.
	\item We can theoretically evaluate the bias under different distributions of the covariates.
\end{itemize}

The theoretical bias results of Section~\ref{sec:theory} provide several anchors for future work. Considering the setting of two uniformly distributed covariates: if $\beta_1$ and $\beta_2$ have the same sign then 
the CATE for $x_1=x_2$ sees the greatest bias, while $x_1\neq x_2$ sees the bias reduced. If the $\beta$s have different signs, the setting is reversed. Knowing these patterns of bias is suggests a natural future direction for algorithm development. In particular, it is possible to mitigate these adverse effects by one of two approaches: first, one can augment the algorithm to perform back-track steps (this would allow covariates to be returned into the potential pool of covariates to drop in line 5 of Algorithm 1). This would allow for multiple estimates of the effect for a single covariate combination --- further combining these will likely produce a more efficient estimate. A second approach allows for using the FLAME technique to construct a hierarchical Bayesian model for the CATEs within each bin. This approach can leverage information about easily estimated CATEs using many covariates in order to smooth estimates of harder-to-estimate CATEs without requiring a model for the outcome.

Further generalizations of FLAME can accommodate continuous and other high dimensional covariates. A natural approach for continuous covariates coarsens them to discrete ones and adds them to the existing framework. However, drawbacks of such an approach are that it throws away information during coarsening and that coarsening cannot be accomplished automatically. An alternative approach can leverage the natural metric associated with many continuous and high dimensional covariates by requiring matches in FLAME to be close in that metric. These continuous covariates can be subjected to a similar dropping scheme as FLAME, while tuning the closeness parameter provides a trade-off between the importance of discrete and continuous information. These are ongoing research areas for the authors.

Given FLAME's large benefits in scalability for massive data, parallelization is a clear future direction. Its SQL queries already handle datasets that do not fit in memory, but we may be able to create a faster parallel version of FLAME that takes advantage of the geometry of the matching problem. For instance, FLAME's loop over covariates at each iteration can be split among processors, some of its later computations done, and joined afterwards, all using efficient SQL queries. FLAME's design inspiration comes both from statistics (matching as exactly as possible) and computationally efficiency (efficient SQL queries). It is part of a next generation of statistical techniques that are explicitly designed for use on huge datasets that take advantage of modern computational machinery. 

%Code implementing the FLAME algorithm as well as the examples in this paper is available on the authors' website: \url{https://github.com/ty-w/FLAME}.%%%EDITED FOR BLINDED VERSION OF PAPER! UNBLIND LATER!
% It is likely that more matching techniques in the future will be designed to handle massive datasets with tools from database computation.

% \begin{itemize}[leftmargin=*]
% \itemsep0em
% 	\item How bad is being greedy? Robust worst case. Wondering if we need to have a constraint on match quality and just optimize prediction.
% 	\item Streaming version - can insert exact matches anywhere in the hierarchy easily, but can't change the hierarchy easily.
% 	\item More database stuff?
% \end{itemize}

% \section{Future Work}\label{sec:futurework}
% \sudeepa{this may not go to the paper}
% \begin{enumerate}
% \item \red{How biased are ATT or ATE when we remove features - this should depend on the quality of features we remove?}
% \item \red{How much does prediction ability change when we remove features?}
% \item \red{Asymptotically - we are ok since the state space is finite when p is fixed. What about when p increases? Bound uses minimum of overlap - how overlapped things are. Simple combinatorics. (Need to take into account different numbers of categories - think about it as continuous.)}
% \item \red{How bad is being greedy? Robust worst case. Wondering if we need to have a constraint on match quality and just optimize prediction.}
% \item \red{Streaming version - can insert exact matches anywhere in the hierarchy easily, but can't change the hierarchy easily.}
% \item \red{Bias/variance tradeoff -- relationship to coarsened exact matching}
% \item \red{Load balancing among processor}
% \end{enumerate}

==> flame-full.tex <==

\subsection{FLAME's Full Pseudocode} \label{sec:flame-full}
% The full pseudocode for FLAME is in the supplement, in Section \ref{sec:FLAMEPseudocode}. There are several adjustable parameters in FLAME, including whether we use units with replacement or without replacement, the minimum number of treatment and control units in each valid group, the parameter trading off $\PE$ and $\BF$, the cutoff for when to stop matching (and remove the remaining outliers), and whether units can be used more than once (with or without replacement). FLAME's performance does not seem to be very sensitive to these parameter values, but they are important for interpretability. 
In this section, we describe a more detailed version of FLAME as an approximate solution to the Full-AEMR. Our implementations and experiments are developed based on the framework of this section. We begin by introducing the objective \totalMQ\, as an auxiliary objective for FLAME's implementation. 

\textbf{Match Quality as the Efroymson's Criterion:}
%}\label{Subsec:MQ}
The input is the data table $D$, a holdout training dataset $D^H$, 
%matching covariates $X$ (indexed by $J$), treatment indicator $T$, outcome variable $Y$ 
and the Efroymson's criterion: match quality $\MQ$. If $\MQ$ is large, it means enough covariates have been retained to predict well on the hold-out training set, and that the balance between treatment and control is sufficient. The algorithm's goal is to determine the selector indicators, denoted by $\Theta$, which choose a subset of rows (units) and columns (covariates) of $D$ and $D^H$ that are available when $u$ is matched, \ie, 
%$\Theta: D,u \rightarrow$ rows of $D$ and columns of $D$ and $D^H$ to use at the time when $u$ is matched: 
%$\Theta(D, u)=(\textrm{rows}_{\Theta,u},\textrm{columns}_{\Theta,u})$. We denote 
$D_{\Theta,u} = D(\textrm{rows}_{\Theta,u},\textrm{columns}_{\Theta,u})$ denotes the dataset available when $u$ is matched. 
Here $\textrm{rows}_{\Theta,u}$ denotes the set of units that have not yet been matched at the iteration when $u$ is being considered for matching, and $\textrm{columns}_{\Theta,u}$ denotes the set of available columns that will be used to match $u$. 
For the holdout training set (discussed further in what follows), we use the same set of available covariates when $u$ is matched but use the full set of training rows, \ie, $D^H_{\Theta,u} = D^H(\cdot,\textrm{columns}_{\Theta,u})$.  
%The number of unmatched units, which do not belong to any valid matched groups satisfying properties (R1)-(R5) when the execution of FLAME is over,  is denoted by $\#\textrm{unmatched}$. %\red{??$=|\# u:\Theta(D,u)\rightarrow\emptyset|$??}.  

%The  generic framework %FLAME algorithm %approximately
FLAME aims to complete the variable selection task. In other words, learn the selection indicators $\Theta$. These selectors  determine the matching process; once the selector function is chosen, $u$ is matched according to the other units that are available when the selector function says that $u$ will be matched, with the covariates that are available at that time. At a timestep $t$, the FLAME's Efroymson's criterion is 
%FLAME focuses on $\Theta$'s that are of a certain form: 
\begin{align} \label{equn:mq2} 
 \mathrm{\texttt{MQ}} = - \PE(D^H_{\Theta,u}) + C \times \BF(D_{\Theta,u}), %+C' \times \Penalty(\#\textrm{unmatched}).
\end{align}
where $C$ trades off between \texttt{PE} and \texttt{BF}. 
% \begin{align*}
% \min_{\Theta} \sum_{u=1}^n \PE(D^H_{\Theta,u}) , \text{ subject to } &\sum_{u=1}^n \BF(D_{\Theta,u}) \ge \epsilon. 
% \end{align*}
%Here, \Penalty\ is a function whose input is an integer, which is the number of unmatched points, and returns a real number. Inclusion of \Penalty\ agrees with goal (R4), which is to keep the number of unmatched units small.
% The function $\BF(D_{\Theta,u})$ is a \emph{balancing factor}. 
% that is constrained to be larger than a threshold $\epsilon$. 
%maximized when the largest possible fractions of treatment and control populations are matched. 
%This helps with goal (R4), which is to keep the number of unmatched units small. This also helps with goal (R2), which is that throughout the procedure, as many covariates as possible should be used for defining matched groups. This is due to the fact that the %FLAME algorithm 
%framework drops a variable from consideration only when a unit cannot be matched in a valid group satisfying (R1) considering the set of all available covariates. 
Function $\PE(D^H_{\Theta,u})$ is the \emph{prediction error}, which ensures that the set of covariates available when units are matched is sufficient to maintain prediction quality.
% (the example 2\% was used in Section~\ref{sec:flame-framework}). 
FLAME can use any machine learning model on the hold-out training set to produce $\PE(D^H_{\Theta,u})$. In practice, one should choose a model that generalizes well to compute $\PE(D^H_{\Theta,u})$. In our own experiments, linear regressors and decision trees are used as the models for computing $\PE(D^H_{\Theta,u})$. %Using the Lagrangian relaxation, we rewrite the objective as follows: 
% \begin{align}
% %\lefteqn{
% %\min_{\Theta} \PE(D^H_{\Theta,u}) , \\
%  %\text{ where}}
% \lefteqn{\max_{\Theta}\totalMQ(D,D^H,\Theta), \text{ where}} \nonunmber\\
% %\label{equn:opt}
% \totalMQ(D,D^H,\Theta)&=&%\sum_{u=1}^n \MQ(D_{\Theta,u},D^H_{\Theta,u})\label{equn:mq1}=%\\ %+ \Penalty(\#\textrm{unmatched})\\
% %&=&
% \sum_{u=1}^n [- \PE(D^H_{\Theta,u}) + C \times \BF(D_{\Theta,u})] \label{equn:mq2} %+C' \times \Penalty(\#\textrm{unmatched}).
% \end{align}

A lower prediction error is better, so $\PE$ is negated in (\ref{equn:mq2}) since we are maximizing the total matched quality. We define these below, using our class of selector functions $\Theta$. In (\ref{equn:mq2}), $C$ is a trade-off parameter between the balancing factor and the prediction error. 
%Note that (R1) is always guaranteed because we will not match any treated 
% (or control) 
%unit unless there is a corresponding control 
% (or treated) 
%unit in the matched group. 
%and $C'$ are tradeoff parameters between the goals (R2), (R3) and (R4).

\textbf{FLAME Iterations:~} 
For FLAME, the Efroymson's criterion (\ref{equn:mq2}) gives a sequence of selection indicators $\Theta$. These indicators $\Theta$ sequentially reduce the number of rows and columns used for matching. We use $\Theta (j)$ to denote the covariate that is eliminated in the $j$-th iteration. 
% It eliminates covariates according to a partial permutation $\pi$ over the indices of the covariates $J = \{1, \cdots, p\}$. For a unit $u$ and a subset of indexes $J' \subseteq J$ of covariates, let $X(u, J')$ denote the value of the covariates matching the indexes in $J'$. 
% \par 
At iteration $\iter-1$, FLAME has dropped covariates $\Theta(1)$, $\Theta(2)$, .., $\Theta(\iter-1)$. Thus, the set of remaining covariates at time $\iter$ is $J \setminus \{ \Theta (j) \}_{j=1}^{l-1}$. 
At iteration $\iter$, if $u$ has not already been matched, and if there is an exact match for unit $u$ on the covariates that remain, then $u$ is matched at iteration $\iter$, and its $\MQ$ comes from iteration $\iter$. 
Said another way, consider conditions: (a) $u$ has not been matched before $\iter$, i.e., there is no $k$ satisfying condition (R1) such that \[X(u, \JJ) = X(k,\JJ);\] (b) $u$ is matched at $\iter$: $\exists$ $k$ satisfying (R1) (\ie, $T_u = 1 - T_k$) such that \[X(u, \JJ) = X(k,\JJ).\]
% \begin{itemize}
% \item (a) $u$ has not been matched before $\iter$, i.e., there is no $k$ satisfying condition (R1) such that 
% \[X(u, \JJ)=X(k,\JJ).\]
% \item (b) $u$ is matched at $\iter$: $\exists$ $k$ satisfying (R1) (\ie, $T_u = 1 - T_k$) such that \[X(u, \JJ)=X(k,\JJ).\]
% \end{itemize}
If (a) and (b) hold for unit $u$, then $u$ is matched at iteration $\iter$. Define $M_u$ to be the iteration at which $u$ is matched: $M_u=\iter$ such that (a) and (b) both hold at $\iter$. If $u$ is never matched ((b) never holds for any $\iter$ before the stopping iteration $T$), then set $M_u=\infty$. Thus, when $M_u=\iter$, the columns of data used to match $u$ are: $\textrm{columns}_{\Theta,u}=\JJ$.

The balancing factor and predictive error of a unit $u$
%FLAME's values for $u$'s  
depend only on the data available in the iteration when it is matched, and are the same for all $u$ matched at that iteration. 
% Normalizing by the number of units matched in level $\iter$, denoted by $n_{\iter}$, the balancing factor and predictive error of a unit $u$ are: $\BF(D_{\Theta,u})=\frac{\BF(D_{\Theta,(\iter)})}{n_{\iter}}$ and $\PE(D_{\Theta,u}^H)=\frac{\PE(D_{\Theta,(\iter)}^{H})}{n_{\iter}}$, where  $\BF(D_{\Theta,(\iter)}), \PE(D_{\Theta,(\iter)}^{H})$ are the balancing factor and predictive error at level $\iter$. This simplifies expression (\ref{equn:mq2}) to: 
% \begin{equation}\label{equn:opt-level}
% \MQ(D,D^H,\Theta)= \sum_{\iter \geq 1} [- \PE(D^H_{\Theta,\iter}) + C \times \BF(D_{\Theta,\iter})].
% \end{equation}
For \BF, it is desirable that each dropped set of covariates maximizes the fraction of matched individuals from the available pools of units. If $\BF$ is high in earlier iterations, more of the matched units will exactly match on almost all covariates (in agreement with (R2)). We write this as follows (\#\ denotes `the number of'): 
% {\small
 \begin{eqnarray}
BF(D_{\Theta,(\iter)}) %\hspace*{-5pt} 
 &=
\frac{\sum_u 1_{T_u=0,M_u=\iter}} { \sum_u 1_{T_u=0,M_u\geq \iter}}
+
\frac{ \sum_u 1_{T_u=1,M_u= \iter} }{ \sum_u 1_{T_u=1,M_u\geq \iter}} \nonumber \\
&= \frac{ \text{\# matched control}}{\text{\# available control}} + \frac{\text{\# matched treated}}{\text{\# available treated}} 
\label{equn:BF}
 \end{eqnarray}
% }

%{\small
%%%% Old one with 
% \begin{eqnarray}
%BF(D_{\Theta,(\iter)})&\hspace*{-5pt}=& \frac{\text{\# available control} - \text{\# matched control}}{\text{\# available control}} + \frac{\text{\# available treated} - \text{\# matched treated}}{\text{\# available treated}}\nonumber\\
%& = &\frac{
%\sum_u 1_{T_u=0,M_u\geq \iter}-
%\sum_u 1_{T_u=0,M_u=\iter}}
%{
%\sum_u 1_{T_u=0,M_u\geq \iter}}
%+\frac{
%\sum_u 1_{T_u=1,M_u\geq \iter}-
%\sum_u 1_{T_u=1,M_u= \iter}}
%{
%\sum_u 1_{T_u=1,M_u\geq \iter}}.
%\label{equn:BF}
% \end{eqnarray}
%}

If we choose covariates to drop using only $\BF$, we may omit covariates that are important for maintaining prediction quality, which could ruin the results of our matching procedure. To counteract this, we associate the matching assignment with the outcome as well as with the treatment assignment \citep[see also][]{rubin1996matching,brookhart2006variable}. A natural approach for this considers a holdout training set $D^H=[X^H, Y^H, T^H]$ that includes both treatment and control units for which predictive quality (predictive error \PE) can be measured. Here we can, for example, use only the covariates available at iteration $\iter$, and $\beta_0$ and $\beta_1$ are vectors of that same size, representing the coefficients obtained by linear regressions on control and treatment units:
%naively via least squares on \red{test data (?)}: \sudeepa{normalization}
\begin{align}
%R^{\textrm{test}}(X^H,Y^H)&=&
\PE(D^H_{ \Theta,(\iter)})  &=
\min_{\beta_0,\beta_1}\left[ 
\frac{1}{\sum (1-T^{H}_u)}\sum_{u:T_u^{H}=0} \left(Y_u^H - \hat{Y}_u^H \right)^2 \right. \nonumber  \\
&+ \left. \frac{1}{\sum T^{H}_u}\sum_{u:T_u^{H}=1}\left(Y_u^H - \hat{Y}_u^H \right)^2 \right], \label{equn:PE}
\end{align}
where $\hat{Y}_u^H = X^H\left(u,\JJt \right)\beta_T $, and $T \in \{0,1 \}$ is the treatment indicator. 
The weighted combination of (\ref{equn:BF}) and (\ref{equn:PE}) is our match quality measure \MQ. The prediction error \PE\; is essentially a measure of predictive power of a given subset of covariates. This measure does not need to depend on 
% linear regression or 
any specific machine learning model, which makes FLAME less model-dependent. For instance, one can replace \PE\; with a classification metric if desired. 

With the definitions above, selector function $\Theta$ is uniquely defined by the partial permutation $\pi$, which is a reordering a subset of indices $1,..,J$. For instance, $\pi$ might have FLAME drop coefficients $6,13,2,8$ in that order and then keep the remaining coefficients, leaving some units unmatched. Overloading notation, our goal is thus to maximize:
\[\max_{\pi}\totalMQ(D,D^H,\pi).\]
(This notation is overloaded since $\pi$ tells us only the order in which covariates are removed. FLAME's matching procedure, defined above, is now implicit from this notation.) 

Global optimization of total match quality $\totalMQ$ with respect to partial permutations $\pi$ requires a search over a space that is exponential in the number of covariates, since it requires the choice of a subset of covariates and order of covariates to remove. We instead use a backwards elimination procedure, where we choose the optimal covariate to eliminate at each iteration and optimize parameters in between eliminating covariates. This will allow the method to scale to a huge number of covariates and observations. We have reason to believe that in many cases, the solution FLAME finds is not too far from optimal; it tends to protect features from elimination that are important for prediction or match quality, and the exact order in which the less relevant features are removed does not tend to be important. 

For FLAME, $\pi(\iter)$ is computed at iteration $\iter$ of the algorithm by performing linear regression on the holdout training set to determine the next feature to drop for backwards elimination. Each remaining feature is checked, and the one that least damages prediction quality is chosen for removal, and that is $\pi(\iter)$.

\textbf{Early stopping:} While FLAME aims to remove irrelevant covariates, it will ultimately starts to remove relevant covariates and introducing bias. If no early stopping condition is imposed, one should extract the FLAME result in a hindsight fashion - run to the end and exact the \MQ\  on each level. As illustrated in Figure \ref{fig:flame-mq}, there is a sudden drop in \MQ , typically when FLAME starts to remove relevant covariates. A rule of thumb is to use results before the drop of \MQ. 


\textbf{Pseudocode of FLAME:} To summarize, the above procedure is described in Algorithm \ref{algo:basic-FAME} as a generic algorithm called \texttt{FLAME-Generic} (for matching without replacement). \texttt{FLAME-Generic} critically uses a subroutine \BasicExactMatch\ to find matches for different units, which is elaborated in more detail in Algorithm \ref{algo:basicExactMatch}. For matching with replacement, we work with the original dataset in each iteration (i.e., do not remove matches inside the while loop before the next iteration starts). Further, we keep track of the main matched groups for units when they are matched for the first time.  

==> introduction.tex <==
% !TEX root = main.tex
\section{Introduction}\label{sec:introduction}

Questions of robust causal inference, beyond simple correlations or model-based predictions, are practically unavoidable in %various domains like 
health, medicine, or social studies. Causal inference goes beyond simpler correlation, association, or model-based predictive analysis as it attempts to estimate the causal effects of a certain intervention. In the context of the clinical intervention, we are interested in how the binary treatment intervention strategy causes the outcome to change. 
%Causal inference is a foundation for policy-making.
%If the strategy is only associated with a reduction in infection rate, then its use in a different setting could lead to no effect, or worse, a reverse effect. 

%In the context of the potential outcomes framework \citep{Neyman1923,rubin1974estimating,holland1986statistics,rubin2011causal}, we consider a two arm intervention $T$, including one \emph{treatment} ($T=1$) arm and one \emph{control} ($T=0$) arm. The crux of the potential outcomes framework is introducing the two potential outcomes $Y_i(0)$ and $Y_i(1)$ for unit $i$ in the study. $Y_i(0)$ represents the outcome had the unit been exposed to the control arm and $Y_i(1)$  represents the outcome had the unit been exposed to the treatment arm. The curse of causal inference is that only one of the two potential outcomes can be observed for each unit. A secondary difficulty arises when considering the differences between randomized experiments and observational studies \citep{ImaKinStu08misunderstanding}.
%\emph{Randomized experiments} are frequently treated as a gold standard for causal inference. Consider estimating the \emph{Average Treatment Effect (ATE)}: $\frac{1}{n}\sum_{i}(Y_i(1)-Y_i(0))$, where $Y_i(1)$ and $Y_i(0)$ are the potential outcomes for unit $i$. %In the simplest setting, a randomized experiment is carried out by assigning units to treatment and control units completely at random. Under the \emph{Stable Unit Treatment Value Assumption (SUTVA)}, where there is only one type of treatment and only one type of control and the treatment of unit $i$ only affects the outcomes of unit $i$ (this is known as the \emph{Individualistic Treatment Response} assumption in \cite{manski2013identification}), this assignment mechanism leads to the following unbiased estimate of the ATE: 
%\begin{equation}
% \small{\widehat{ATE} = \frac{1}{|\{i:T_i=1\}|}\sum_{i:T_i=1}Y_i^\obs - \frac{1}{|\{i:T_i=0\}|}\sum_{i:T_i=0}Y_i^\obs}.
%\label{eq:atehat}
%\end{equation}
%The setting of randomized experiments becomes much more complicated when SUTVA is violated. This has led to a large literature on interference, the notion that the treatment of individual $i$ can affect the outcome of individual $j$ \citep{rosenbaum2012interference,sobel2006randomized,tchetgen2012causal,hudgens2008toward}. In particular, much of the recent work has concentrated on experiments where the interference is informed by an underlying network. 
%In \emph{network randomized experiments} the goal of the experimenter is to define both a randomization scheme and an estimand of interest for which the randomization scheme is meaningful. Graph cluster randomization has been used when estimating total treatment effects \citep{ugander2013graph,eckles2014design}. Peer encouragement designs have been used to study peer effects (effects such as treating $j$ and not $i$ on the outcome of $i$), in large social networks \citep{bakshy2012social,eckles2016estimating}. Estimating the standard average treatment effect has been addressed by \cite{jagadeesan2016graphcolor} by describing a restricted randomization scheme. Model-based approaches have been employed to address issues such as network-correlated outcomes \citep{basse2015optimal}. 
%\vspace{-3mm}
%\subsection{Observational Studies and Matching}
While randomized trials are considered the gold standard for causal inference \citep{rubin2008objective}, much of the available data in the clinical and social sciences is observational. 
In such situations, individuals may select into treatment: people who benefit more from pain relievers tend to take them more often, individuals who are likely to succeed in higher education are more likely to enroll in it, and so forth. 
Estimating causal effects in an observational setting becomes a problem of representing the available data as if individuals were assigned to treatment randomly. 
A major benefit of randomization is the covariate balance that it creates between treated and control units. A natural approach to observational studies is the matching of treated and control units such that underlying background covariates are balanced \citep{chapin1947experimental,greenwood1945experimental}. 
In general, the covariate balancing property of matching methods provides a path to proper estimates of causal effects. 

Matching increases the interpretability of causal analyses in several ways. In particular, matching highlights issues with overlap between treatment and control populations, allowing for a careful analysis of why some individuals are treated and others are not. This helps us to find the source of uncertainty in the causal estimates, and helps determine what type of additional data must be collected. Exact matching approaches where individuals are matched on raw covariate values further allows the practitioner to interpret causal estimates within matched populations as conditional average treatment effects. This provides a more granular causal analysis that can provide crucial information on who benefits from treatment most and where resources should be spent for future treatments. Matching can also provide explanations for treatment effect estimates in a way that pure modeling methods (that do not use matching) cannot. 

Early approaches to matching considered exact matching on covariates but quickly ran into issues of insufficient sample size when the number of covariates was even moderately large; each matched group must include one treatment and one control observation, and in high dimensions, the matches simply do not exist. 
In the 1970's and 1980's, a large literature on different dimension reduction approaches to matching was developed \citep[e.g.,][]{rubin1973matching,rubin1973use,rubin1976multivariate,cochran1973controlling} with the extreme being work on propensity score matching, which was later extended to work on penalized regression approaches that leverage propensity \citep{schneeweiss2009high,rassen2012using,belloni2014inference,farrell2015robust}.
The problem with propensity score methods is that they require a proper specification of either the propensity score model or the outcome model, neither of which is true in practice. The doubly robust literature allows for only one of the two models to be specified correctly, but there is no reason that either of these models would be specified correctly in practice.
% are that it is both computationally inefficient (because it requires fitting models) and statistically inefficient. \textcolor{red}{Explain why - is it because it makes strong assumptions that are violated?}
 
%One of the most prevalent approaches in current research is the propensity score, the distribution of treatment assignment conditional on background covariates. 
%In propensity score matching, the full distribution of covariates is projected onto only one dimension -- the conditional distribution of treatment assignment given background covariates.
%\textcolor{red}{Need this? \citet{rosenbaum1983central} demonstrated that under mild assumptions the propensity score was a balancing score that allowed for the unbiased estimation of average causal effects. Beyond na\"ive matching, the propensity score has been integrated into subclassification \citep{rosenbaum1984reducing} and multivariate matching schemes \citep{rosenbaum1985constructing} for observational data. } 
%To address these problems, the high dimensional variable selection literature has suggested penalized regression approaches to propensity scores estimation \citep{schneeweiss2009high,rassen2012using,belloni2014inference,farrell2015robust}. Many of these ideas borrow from variable selection and modeling approaches that have been applied to randomized trials where heterogeneous effects are being estimated 
%\textcolor{red}{I left these out}\citep{imai2013estimating,tian2014simple,dasgupta2015causal}.  \cite{king2011comparative}

%Using variable selection approaches, such as the lasso, for high dimensional propensity score models does not overfit the treatment indicator, but does not necessarily produce estimates that are interpretable as balancing scores. \textcolor{red}{ so what? why aren't we just doing this?} 
% If we project onto only one dimension means that units that are dissimilar to each other in every covariate can still be matched. Further in order for the 
%\citep[See King's paper on why we should not use propensity score matching][.]{,king?}

%\vspace{-3mm}
%\subsection{Recent Advances in Matching}
%With the advent of big data, traditional matching tools such as vanilla propensity score methods have become both computationally and statistically inefficient. These needs have led to the 
An alternative technique, coarsened exact matching, creates matches that attempt to preserve more covariate information.  
%recent surge of coarsened exact matching, high dimensional matching and computationally tractable matching approaches. 
It bypasses the need to fit complicated propensity score models by coarsening or discretizing covariates in such a way that the newly constructed covariates allow for exact matching \citep{iacus2011causal,iacus2011multivariate}. This approach is appealing when there are many continuous covariates that are naturally amenable to binning. However, when most or all of the covariates are categorical, coarsening becomes impossible without introducing a calculus on all of the covariates. This can be problematic in high dimensions, and tends to have the same problem as nearest neighbor techniques, which are well-known to perform poorly in high dimensions. Further, when categorical variables have two levels, coarsening is equivalent to variable selection. In this setting, coarsened exact matching would lead to the same matches as high dimensional propensity score techniques with variable selection.


A similar problem exists with what is called ``optimal" matching in the literature \citep{rosenbaum2016imposing}. A distance metric over variables is defined manually, which introduces a calculus on the covariates. That distance metric is used as input to a network flow problem which optimizes match quality. Despite the optimality of the solution network flow problem, the quality of the matches is questionable since it relies on a manually defined distance measure. Network flow problems also cannot directly handle constraints, the user needs to manually manipulate the algorithm in order to obtain desired balance constraints \citep{zubizarreta2012using}.
%Exact matching, though not possible in high dimensions, would be a gold standard for coarsened exact matching.



% \subsubsection*{C.1.2.2: High dimensional matching}
% \cite{,bottou2013counterfactual,,,hu2014estimation,,,rubin2000combining,,}

% \subsubsection*{C.1.2.3: Computationally tractable matching}
%To avoid penalization and to produce matches that assist in unbiased and low variance estimation of causal estimands, computational machinery from the optimization literature has been introduced. In particular, a new  matching scheme has been developed that 

The problems with network flow optimization highlight an important concern about non-exact matching methods generally, which is that they implicitly approximate the solution of a hard combinatorial optimization problem. It is possible that high quality match assignments exist, but the standard approximate methods of constructing matches, such as network flow optimization did not find them. To handle the problem of finding suboptimal match assignments, some newer matching schemes use mixed integer programming, which is a flexible framework that can accommodate linear balance constraints \citep{zubizarreta2012using,zubizarreta2014matching,keele2014optimal,resa2016evaluation,AlamRu15,AlamRu15nonparam}.
%These matching algorithms are possibly the best options available currently for obtaining unbiased, low variance estimators of the treatment effect. 
However, these methods have two major disadvantages: first they cannot scale to even many modestly-sized problems; second, they may be trying to match units on covariates that are not important in any way. 

%takes advantage of linear balance constraints for the covariates of interest \citep{zubizarreta2012using,zubizarreta2014matching,keele2014optimal,resa2016evaluation,NoorEAlamRu16}. This approach uses mixed integer linear programming (MIP) and is computationally expensive, but it would (given possibly exponential computation time) compute the best possible set of matched pairs with optimal covariate balance. Since the methods use MIP software, they are designed for high-quality, smaller scale experiments, and cannot reasonably be used for very large-scale experiments. 



%Much of massive health records data comes in the form of categorical variables -- be they demographic information such as sex, race, and education level, or clinically informative variables such as smoking status, depression scale, or previous medical conditions. To properly analyze clinical outcomes in observational studies it is desired to construct control and treatment groups that are well balanced on background covariates. In order to define ``good balancing'' or ``good matching'' one first must determine a calculus on the categorical variables. That is, one must define a metric $d(\cdot,\cdot)$ that takes high dimensional covariates $X$ and $Y$ as its argument. While many different metrics have been discussed in the literature (such as propensity score matching \citep{rosenbaum1983central}, Mahalanobis distance matching \citep{rubin1992characterizing} and coarsened exact matching \citep{iacus2011causal} among others), the simple exact matching setting where $d(X,Y)=0$ if $X=Y$ and $d(X,Y) = \infty$ otherwise has both statistical and analytical advantages \citep{ImaKinStu08misunderstanding}. 


%\subsubsection{Fast Large-scale Almost-Matching-Exactly (FLAME) Algorithm using As Much Data As Possible}Exact matching is an observational study equivalent to randomized experiment blocking \citep{ImaKinStu08misunderstanding} though it comes with several additional assumptions. In particular, the balance in a matched sample by definition happens with already collected data. When the collected data are limited this can lead to poor matches (e.g., matched groups do not contain both treated and untreated units), or to potential biasing of estimated effects in cases where the matching variables are poorly associated with outcome variables and treatment indicators. Modern data streams and computational tools have the potential of avoiding these problems by matching exactly on a much larger collection of variables (unlike for example in \cite{chapin1947experimental} where only six categorical variables were available). For example, the %2010 Natality Public Use File provided publicly available \emph{natality dataset} of 2010 \footnote{This dataset is available from the National Center for Health Statistics (NCHS) through the Centers for Disease Control and Prevention (CDC): \url{http://www.cdc.gov/nchs/data_access/ftp\_data.htm}}, which contains all the births registered in the United States in 2010, includes over four million anonymized records for 233 demographic and clinical variables. Similarly, the public-use portion of the \emph{AddHealth Wave I dataset} \footnote{This dataset is partially funded by the NIH and is available from the University of North Carolina, Chapel Hill: \url{http://www.cpc.unc.edu/projects/addhealth/documentation/publicdata}} contains 2,801 mostly categorical variables about 6,504 individuals (the restricted use version of the dataset includes over 20,000 individuals).
%Massive datasets such as these lead to a new problem with exact matching --- even with millions of observations it is very likely that most units will be unmatched or matched only to units with the same treatment indicator. 
%\par
%The overarching approach to overcoming these issues revolves around different coarsening methods. Propensity score approaches distill the information in the covariates into a single number and match solely based on it. In order to deal with large numbers of covariates, regularized propensity score methods have been proposed. Coarsened exact matching (CEM)  requires ``substantive knowledge of the measurement scale'' to bin continuous covariates which are then exactly matched; and while a default approach is available, it is extremely sensitive to bin boundaries \citep{iacus2011causal}. Combining nominal categorical variables using an approach like CEM is discouraged unless very specific user specification is provided and no default approaches are available. 



%\subsubsection{Parallel Implementation with Large Number of Covariates}
%red{TODO for Sudeepa: we need a section on \url{https://dev.mysql.com/doc/refman/5.7/en/column-count-limit.html} that discusses that SQL server can't deal with this --- we can make the point later in section 4 of how we solve this problem with a fancy tree-like algorithm}

In this work, we avoid the introduction of traditional regularization or a measurement scale on the covariates, and instead propose a data-adaptive approach to almost-exact matching. Our method (FLAME - Fast, Large-scale, Almost Matching Exactly) creates matches that include as many covariates as possible, and iteratively drops covariates that are successively less useful for predicting outcomes. It takes into account an aspect of large samples that past work does not: how to retain as much information as possible when matching, by constructing matches on partial information. This allows the matches to be almost exact, which helps with interpretability, and retains as much important information as possible within each match. It improves over coarsened exact matching in that it does not introduce a distance metric on covariate space \textit{a priori}, since our distance metric is adaptive. It improves over regression and propensity methods in that it does not force a model form, instead it tries to match on covariates almost exactly. It improves over network flow formulations in that it considers covariate balance in the formulation. 
It improves over mixed integer programming methods in that it considers only variables it deems to be important, and scales nicely with the sample size and number of covariates. 

By dropping covariates, FLAME increases bias in order to make predictions of conditional average treatment effect. We can actually calculate FLAME's bias directly in some cases, and its bias depends directly on how important the dropped covariates are to predicting the output. If only the irrelevant covariates are dropped, the estimates are unbiased. In that case, FLAME's estimates and the gold standard estimates of exact matches are identical.

A major benefit of FLAME is that it lends naturally to fast implementations for extremely large datasets. 
FLAME has two implementations: one that uses bit vectors, which is extremely fast for data that has been preprocessed and fits in memory. The other implementation leverage database management systems (e.g., postgresql \citep{postgresql}), which has highly optimized built-in SQL \emph{group-by} operators, can operate directly on the database, and does not require the data to fit in memory. Only a few lines of SQL code are needed to perform matching, and the use of database systems makes the matching algorithm better suitable for parallel executions.

%-----------begin added Aug3 by Tianyu---------------% 
%FLAME meets the congruence principle \citep{mielke2007permutation}. The congruence principle states that when the data space and the matching space are the same, the result tends to be more robust and intuitive. The majority of matching method violate this principle by either a logistic transformation or a Mahalanobis transformation of the data space, whereas FLAME naturally satisfies this principle.

%-----------end added Aug3 by Tianyu---------------% 

%\subsection{Database Queries for Efficient FLAME Implementation}
% Arguably the hardest part of exact matching with a large number of variables is the actual construction of the groups. Different database management schemes contain built in grouping functions. \todoC{For Cynthia/Sudeepa: describe SQL group by as dplyr group\_by approaches. We propose to take advantage of the built in capabilities of these database structures in order to improve computation.}
%Arguably the hardest part of exact matching with a large number of variables is the actual construction of the groups. There are a number of matching libraries that support different matching functionality more efficiently than the inbuilt methods in R or Python. One of the novel directions in the proposed project is the use of 
%FLAME leverages
%\emph{Database Management Systems} (like 
%\cite{msftsql}
% Microsoft SQL Server
% \footnote{Documentation for Microsoft SQL Server is available at: \url{}} 
%or \cite{postgresql}
% \footnote{Documentation for PostgreSQL is available at \url{https://www.postgresql.org}}
%) and \emph{SQL queries}.
% to develop efficient and scalable matching algorithms for big observational datasets having a large number of records as well as a large number of fields. 
%The highly optimized built-in SQL \emph{group-by} operators supported by these database systems can compute exact matches on a given set of covariates with a few lines of SQL code. Our 
%Further, unlike popular matching packages like MatchIt \citep{matchit2011}, these database systems do not require the data to be loaded into memory first (which is difficult and takes additional pre-processing time for big datasets), and using database systems makes the matching algorithms better suitable for parallel executions. 
%To move away from dependence on available main memory, one must introduce an interface between the analytic software and a database structure\footnote{There is movement in this direction with Microsoft building an R interface for their SQL server as well as R packages such as DPLYR that can natively interface with certain databases.}. 
%In this project, we will explore how database systems and SQL queries can help in selection of covariates that result in a matching with high quality while utilizing as many input records as possible. We will produce R packages that address these needs and implement a flexible version of the FAME algorithm. 


In what follows, we first introduce FLAME's framework of iteratively dropping covariates (Section \ref{sec:fame-framework}). We then discuss FLAME's algorithms and implementations (Section \ref{sec:algorithms}), provide experiments (Section \ref{sec:experiments}), and a precise theoretical calculation of FLAME's statistical bias (Section \ref{sec:theory}). A general introduction to matching methods is that of \citet{stuart2010matching}. 

% The goals for this project build on each other. Broadly, Goals 1 (formalizing match quality measure), 2 (information bounds to justify the choice of match quality measure) and 4 (causal estimands the FAME can help estimate) address the statistical methodology and theory; Goals 3 (polynomial time relaxation of the algorithm) and 5 (fast implementation of exact matching) address the Computer Science theory; Goal 6 describes possible extensions in both the statistical and CS directions. Clinical Relevance is described at the end.  
%The general question of match quality has been open in statistics since the introduction of non-exact matching methods. Common methods of assessing balance consider a direct measure of similarity between the covariates for treated and control units. For example, the ``Love plots'' of \cite{ahmed2006heart} plot normalized differences in means between treated and control units for each covariate before and after matching (this is a graphical representation of standardized bias of \cite{rosenbaum1985constructing}). This and other graphical measures such as quantile-quantile plots and weighted boxplots are only meaningful when the notion of an average is reasonable \citep{joffe1999invited,stuart2010matching}. When considering a propensity score approach to matching \cite{rubin2001using} recommends assessing the differences in mean and variance of the propensity score for the treated and control units. \sudeepa{revived from proposal - need this?}
\par
%However, when considering categorical variables, the natural distance measure between any two vectors is zero if the two vectors of covariates are exactly equal and infinite otherwise. The multivariate imbalance measure of \red{cite} \cite{iacus2011multivariate} considers the difference in the empirical distributions of binned covariates between treated and control units and so a measure of $0$ suggests no overlap while a measure of $1$ suggests overlap. This approach is motivated by coarsening continuous variables and is employed when the number of covariates is not too large. When working with large numbers of nominal variables the multivariate imbalance measure is almost always zero and as such 


%\textcolor{red}{Put this later - do not need to have these in memory -  (unlike, for instance, popular matching packages like MatchIt \citep{matchit2011}).}



==> macros-icml.tex <==
% \newcommand{\red}[1]{{\textbf {\tt {\color{red} [{#1}]}}}}
\usepackage{MnSymbol}
\usepackage{eqnarray}
\usepackage{amstext}
\usepackage{alltt}
\usepackage{blkarray}
\usepackage{amsthm}
\usepackage{enumitem}
\usepackage{makecell}
% \usepackage{xcolor}

%\newcomand{\btheta}{\text{\boldmath$\theta$}}
\usepackage{bm}
\newcommand{\btheta}{\bm{\theta}}

\newtheorem{definition}{Definition} 
\newtheorem{proposition}{Proposition} 
\newtheorem{theorem}{Theorem} 

% \usepackage{algcompatible}

\newcommand{\ie}{{\it i.e.}} %\xspace}
\newcommand{\eg}{{\it e.g.}} %\xspace}

\newcommand{\iter}{{l}}

\newcommand{\BasicExactMatch}{{\tt BasicExactMatch}}

\newcommand{\MG}{{\cal{MG}}}
\newcommand{\mg}{{\tt{mg}}}
\newcommand{\ismatched}{{\tt is\_matched}}

\newcommand{\totalMQ}{{\tt TotalMQ}}
\newcommand{\MQ}{\text{{\tt MQ}}}
\newcommand{\BF}{{\tt BF}}
\newcommand{\PE}{{\tt PE}}
\newcommand{\JJ}{J\setminus \{\pi(j)\}_{j=1}^{\iter-1}}
\newcommand{\JJt}{J\setminus \{\pi(j)\}_{j=1}^{\iter}}
\newcommand{\x}{{\mathbf{x}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\w}{{\mathbf{w}}}
\newcommand{\uu}{{\mathbf{u}}}

% \newcommand{\alex}[1]{{\texttt {\color{magenta} Alex: [{#1}]}}}
% \newcommand{\cynthia}[1]{{{\tt \color{green} Cynthia: [{#1}]}}}
% \newcommand{\tianyu}[1]{{{\tt \color{purple} Tianyu: [{#1}]}}}
 \newcommand{\sudeepa}[1]{{{\tt \color{blue} Sudeepa: [{#1}]}}}

% \newcommand{\red}[1]{{\textbf {\tt {\color{red} [{#1}]}}}}
% \newcommand{\yellow}[1]{{\textbf {\tt {\color{yellow} [{#1}]}}}}
% \newcommand{\scream}[1]{{{\tt \color{red}{\textbf{[{#1}]}}}}}

\newcommand{\cut}[1]{}

==> max-error-not-used.tex <==
\section{Bias bound via max error}

To start with, we list (reiterate) below the assumptions that we make.
\begin{enumerate}
    \item The covariate space is discrete/categorical. 
    \item Non-zero support assumption: for any $(x_1, x_2, \cdots, x_3)$, there exists $\lambda > 0$, such that $ \mathbb{P}_{D^1} [ X_1 = x_1, \cdots, X_d = x_d ] \ge \lambda$ and $ \mathbb{P}_{D^0} [ X_1 = x_1, \cdots, X_d = x_d ] \ge \lambda$ .
    \item The true outcome functions take values only from [0,1].
    \item Our hypothesis class $\mathcal{H}$ is finite and for $h \in \mathcal{H}$, $h$ only takes values from [0,1]. 
\end{enumerate}


% \vspace{1cm}
% For notational simplicity, we restrict our attentions to two-covariate case. Namely, we only have $x_1, x_2$. 

% Let $\mathcal{F}_k$ be the function class for . 

% We sketch some high level ideas

% \subsubsection*{}

Let's say we are interested in the group $(\mathbf{x} \circ \theta)$
We need a bound for: 
\begin{align}
    &\quad \left| \hat{Y}_{S_1}^{m_1} [f^1 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] - \hat{Y}_{S_0}^{m_0} [f^0 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] \right. \\
    &\qquad \qquad \left. - ( \mathbb{E}_{D^1} [ f^1 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] - \mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] ) \right|
    \\
    &\le \left| \hat{Y}_{S_1}^{m_1} [f^1 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] - \mathbb{E}_{D^1} [ f^1 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| + \\
    & \qquad \qquad \left| \hat{Y}_{S_0}^{m_0} [f^0 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] - \mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right|.
\end{align}
In the above equations, $\mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d] = f^0 ( x_1, \cdots, x_d)$ and  $\mathbb{E}_{D^1} [ f^1 ( X ) | X_1 = x_1, \cdots, X_d = x_d] = f^1 ( x_1, \cdots, x_d)$. But for consistency, we tend to use the notations in the above equations.  

Let's say $h$ is a fixed function from the hyperthesis space $\mathcal{H}$ of finite cadinality. 

% 
% \begin{align}
%     h_1 \in \arg \min_h \max_{j} l (h (\mathbf{x}_{i,j_1}^{1}, \cdots,  \mathbf{x}_{i,j_d}^{1} ) , y_i^{1} ), 
% \end{align}
% where $l$ is the Mean Absolute Error (MAE) loss we use on the holdout set. Here $h_1$ is the minimax estimator with the MAE criterion. 

With respect to the holdout sets $S_H^1$ and $S_H^0$, write 
\begin{align*}
    N^1(x_{j_1}, x_{j_2}, \cdots, x_{j_k}) := \sum_{j=1}^{|S_H^1|} \mathbbm{1} [ \mathbf{x}_{i, j_1}^1 = x_{j_1}, \cdots, \mathbf{x}_{i, j_k}^1 = x_{j_k} ] \\
    N^0(x_{j_1}, x_{j_2}, \cdots, x_{j_k}) := \sum_{j=1}^{|S_H^0|} \mathbbm{1} [ \mathbf{x}_{i, j_1}^0 = x_{j_1}, \cdots, \mathbf{x}_{i, j_k}^0 = x_{j_k} ] .
\end{align*}
In words, $N^1(x_{j_1}, x_{j_2}, \cdots, x_{j_k})$ (resp. $N^0(x_{j_1}, x_{j_2}, \cdots, x_{j_k})$) is the number of points in $S_H^1$ (resp. $S_H^0$) whose covariate values at $(X_{j_1}, \cdots, X_{j_k})$ are $(x_{j_1}, \cdots, x_{j_k})$. 

% From the holdout set $ S_H^1 $ 

For a fixed $h \in \mathcal{H}$, a loss function $l$, and a dataset $S$, we write 
\begin{align}
    &\hat{\epsilon}_{\max}^1 ( X_{j_1}, \cdots, X_{j_k} ; h ; S ) =  \max_{\mathbf{x}_i \in S} l (h (\mathbf{x}_{i,j_1}^{1}, \cdots,  \mathbf{x}_{i,j_k}^{1} ) , y_i^{1} ) \\
    % &\hat{\epsilon}^1 ( X_{j_1}, \cdots, X_{j_k} ; h ) = \frac{1}{N^1(x_{j_1}, \cdots, x_{j_k})} \sum_{j=1}^{N^1(x_{j_1}, \cdots, x_{j_k})} l (h (\mathbf{x}_{i,j_1}^{1}, \cdots,  \mathbf{x}_{i,j_k}^{1} ) , y_i^{1} ) \\
    &\hat{\epsilon}_{\max}^0 ( X_{j_1}, \cdots, X_{j_k} ; h; S ) =  \max_{\mathbf{x}_i \in S} l (h (\mathbf{x}_{i,j_1}^{1}, \cdots,  \mathbf{x}_{i,j_k}^{1} ) , y_i^{1} ) 
    % &\hat{\epsilon}^0 ( X_{j_1}, \cdots, X_{j_k} ; h ) = \frac{1}{N^1(x_{j_1}, \cdots, x_{j_k})} \sum_{j=1}^{N^0(x_{j_1}, \cdots, x_{j_k})} l (h (\mathbf{x}_{i,j_1}^{0}, \cdots,  \mathbf{x}_{i,j_k}^{0} ) , y_i^{1} ) . 
\end{align}
The Equations (8), (9) define the max errors of $h$ on the holdout datasets. 

For a fixed $h$, there is one particular point $(x_{j_1}, \cdots, x_{j_k})$ that maximize the true max error.  
By our assumptions (at the beginning of this section), we have with probability smaller than $(1 - \lambda)^{N^1(x_{j_1}, \cdots, x_{j_k})}$ not hitting the max error maximizing point in $S_H^1$, and probability smaller than $(1 - \lambda)^{N^0(x_{j_1}, \cdots, x_{j_k})}$ not hitting the max error maximizing point in $S_H^0$. 

Next, let's focus on the treated population. 

% and dump $(x_{j_1}, x_{j_2}, \cdots, x_{j_k})$ 
% when the context is clear. 

Therefore, with probability at least $1 - (1 - \lambda)^{N^1 \left( x_{j_1}, x_{j_2}, \cdots, x_{j_k} \right) } $, we have 
\begin{align*}
    \mathbb{E} \left[ \hat{\epsilon}_{\max}^1 \left( X_{j_1}, \cdots, X_{j_k} ; h ; S_H^1 \right) \right] =  \hat{\epsilon}_{\max}^1 \left( X_{j_1}, \cdots, X_{j_k} ; h; S_H^1 \right). 
\end{align*}

% Meanwhile, by Chernoff-Hoeffding bound, we get for any $\delta >0$, with probability at least $1 - \delta$, 

% \begin{align*}
%     \left| \mathbb{E}[ \hat{\epsilon}^1 ( X_{j_1}, \cdots, X_{j_k} ; h ) ] - \hat{\epsilon}^1 ( X_{j_1}, \cdots, X_{j_k} ; h ) \right| \le \sqrt{ \frac{\log \delta / 2}{ N^1 (x_{j_1}, x_{j_2}, \cdots, x_{j_k}) } }
% \end{align*}

The max error concentrates to the expected counterpart (very) fast. 


% This minimax absolute error is slightly different from what we did in the code. %Hopefully it's ok. %Remark: an alternative approach is to do a high probability bound, but I'd prefer this minimax error bound. 

% Let's use $y_j^{1} (X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k})$ to denote the $j$-th observation in set $S_H^1$ whose covariate values on $X_{j_1}, \cdots, X_{j_k} $ are $x_{j_1}, \cdots, x_{j_k}$. Let's say there are $J$ such samples in $S_H^1$. 

%$J ( X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} )$ such samples in $S_H^1$. For simplicity, we write $J := J ( X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} )$

Next, for notational simplicity, we write $n^1 := N^1 ( x_{j_1}, \cdots, = x_{j_k} )$ (resp. $n^0 := N^0 ( x_{j_1}, \cdots, = x_{j_k} )$). 
Next, for any fixed $h^1 \in \mathcal{H}$, with probability at least $ 1 - \left( 1 - \lambda \right)^{ n^1 } - \left( 1 - \lambda \right)^{ \left| MG^1 (x_{j_1}, \cdots, = x_{j_k} ) \right| } $, 
\begin{align} 
    &\quad \left| \hat{Y}_{S_1}^{m^1} [f^1 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] - \mathbb{E}_{D^1} [ f^1 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| \\
    &\le \left| \hat{Y}_{S_1}^{m^1} [f^1 | X_{j_1} =  x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] - h_1 (X_{j_1} =  x_{j_1}, \cdots, X_{j_k} = x_{j_k})  \right|  \\
    & \quad + \left| h_1 (X_{j_1} =  x_{j_1}, \cdots, X_{j_k} = x_{j_k})  - \mathbb{E}_{D^1} [ f^1 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| \\ 
    &\le \frac{1}{n^1} \sum_{i=1}^{n^1} \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h^1 \right. ; MG^1 ( x_{j_1}, \cdots, x_{j_k}  ) ) + \mathbb{E} [  \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h^1 ; S_H^1 \right) ] \\
    &= 2 \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h^1 ; S_H^1 \right)
\end{align}   

Similarly, for the control group, we have, for any fixed $h^0 \in \mathcal{H}$, with probability at least 
$ 1 - \left( 1 - \lambda \right)^{ n^0 } - \left( 1 - \lambda \right)^{ \left| MG^0 (x_{j_1}, \cdots, = x_{j_k} ) \right| } $, 
\begin{align} 
    &\quad \left| \hat{Y}_{S_0}^{m^0} [f^0 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] - \mathbb{E}_{D^0} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| \\
    &\le  2 \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h^0 ; S_H^0 \right)
\end{align} 

Taking a union bound, for a finite hypothesis class $|\mathcal{H}|$, we have, for all $h \in \mathcal{H}$, with probability at least 
\begin{align*}
    1 -  | \mathcal{H} | \left( \left( 1 - \lambda \right)^{ n^0 } - \left( 1 - \lambda \right)^{ \left| MG^0 (x_{j_1}, \cdots, x_{j_k} ) \right|   } \right) - | \mathcal{H} | \left( \left( 1 - \lambda \right)^{ n^1 } - \left( 1 - \lambda \right)^{ \left| MG^1 (x_{j_1}, \cdots, x_{j_k} ) \right|  }  \right),
\end{align*}
we have 
\begin{align}
    &\quad  \left| \mathbb{E}_{D^1} [ f^1 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] - \mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ]  \right. \\
    &\quad  - \left. \left( \hat{Y}_{S_1}^{m^1} [f^1 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ] 
     - \hat{Y}_{S_0}^{m^0} [f^0 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} \right) \right| \\
    & \le  \left| \hat{Y}_{S_1}^{m^1} [f^1 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ]  - \mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| \\
    &\quad + \left| \hat{Y}_{S_0}^{m^0} [f^0 | X_{j_1} = x_{j_1}, \cdots, X_{j_k} = x_{j_k} ]  - \mathbb{E}_{D^0} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| \\
    % &\quad + \left| \mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ]  - \mathbb{E}_{D^0} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| \\ 
    % &\le 2 \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h ; S_H^0 \right) + 2 \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h ; S_H^1 \right) \\ 
    % &\quad + \left|  \mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ]  - \mathbb{E}_{D^0} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] \right| \\
    &\le 2 \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h ; S_H^0 \right) + 2 \hat{\epsilon}_{\max} \left( X_{j_1}, \cdots, X_{j_k} ; h ; S_H^1 \right), %+ 2 d_{TV} (D^1, D^0), 
\end{align}
where (21) is because 
\begin{align*}
    \mathbb{E}_{D^0} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ] &= \mathbb{E}_{D^1} [ f^0 ( X ) | X_1 = x_1, \cdots, X_d = x_d ]
\end{align*}
when we are conditioning on all covariates. Here, $h^1$ and $h^0$ are learned from the holdout set. 
